Are Graph Representation Learning Methods Robust to Graph Sparsity and Asymmetric Node Information?

The growing popularity of Graph Representation Learning (GRL) methods has resulted in the development of a large number of models applied to a miscellany of domains. Behind this diversity of domains, there is a strong heterogeneity of graphs, making it difficult to estimate the expected performance of a model on a new graph, especially when the graph has distinctive characteristics that have not been encountered in the benchmark yet. To address this, we have developed an experimental pipeline, to assess the impact of a given property on the models performances. In this paper, we use this pipeline to study the effect of two specificities encountered on banks transactional graphs resulting from the partial view a bank has on all the individuals and transactions carried out on the market. These specific features are graph sparsity and asymmetric node information. This study demonstrates the robustness of GRL methods to these distinctive characteristics. We believe that this work can ease the evaluation of GRL methods to specific characteristics and foster the development of such methods on transactional graphs.

==> preambule/commandes_math.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Ce fichier contient des nouvelles commandes 
% pour faciliter l'écriture des mathématiques
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Ensembles
\let\ensembleNombre\mathbb
\newcommand*\N{\ensuremath{\ensembleNombre{N}}}       % Ensemble des entiers naturels N
\newcommand*\Z{\ensuremath{\ensembleNombre{Z}}}       % Ensemble des entiers relatifs Z
\newcommand*\Q{\ensuremath{\ensembleNombre{Q}}}       % Ensemble des rationnels Q
\newcommand*\R{\ensuremath{\ensembleNombre{R}}}       % Ensemble des réels R
\newcommand*\Complex{\ensuremath{\ensembleNombre{C}}} % Ensemble des complexes C

% Encadrement
\newcommand{\angles}[1]{\left\langle #1 \right\rangle} % ⟨⟩
\newcommand{\braces}[1]{\left\lbrace #1 \right\rbrace} % {}
\newcommand{\bracks}[1]{\left\lbrack #1 \right\rbrack} % []
\newcommand{\pars}[1]{\left( #1 \right)}               % ()
\newcommand{\norme}[1]{\left\Vert #1\right\Vert}       % Norme
\newcommand{\ent}[1]{\left\lfloor #1\right\rfloor}     % Partie entière inférieure
\newcommand{\entsup}[1]{\left\lceil #1\right\rceil}    % Partie entière supérieure
\newcommand{\abs}[1]{\left\vert #1\right\vert}         % Valeur absolue

% Dérivées
\newcommand{\deriv}[3][]{\frac{\mathrm{d}^{#1}#2}{\mathrm{d} {#3}^{#1}}}    % Dérivée non partielle  
\newcommand{\partiald}[3][]{\frac{\partial^{#1}#2}{\partial {#3}^{#1}}} % Dérivée partielle   

% Intervalles
\newcommand*\intervalle[4]{\left#1 #2 \, ; #3 \right#4}                       % Définit la notion d'intervalle
\newcommand*\intervalleOO[2]{\intervalle{]}{#1}{#2}{[}}                       % ]a ; b[
\newcommand*\intervalleFF[2]{\intervalle{[}{#1}{#2}{]}}                       % [a ; b]
\newcommand*\intervalleOF[2]{\intervalle{]}{#1}{#2}{]}}                       % ]a ; b]
\newcommand*\intervalleFO[2]{\intervalle{[}{#1}{#2}{[}}                       % [a ; b[
\newcommand*\intervalleEntier[2]{\intervalle{\llbracket}{#1}{#2}{\rrbracket}} % Ensemble d'entiers

% Ensemble "tel que"
\newcommand*\enstq[2]{\braces{#1,\; #2}}                                      

% Probabilité, espérance, variance, covariance et corrélation
\newcommandx{\proba}[3][1, 3=0]{
\ifthenelse{\isempty{#2}}{\mathbb{P}_{#1}}{%
\ifthenelse{\equal{#3}{0}}{\mathbb{P}_{#1}\pars{#2}}{\mathbb{P}_{#1}\pars{#2 \middle| #3}}}%
}
\newcommandx{\esp}[3][1, 3=0]{
\ifthenelse{\isempty{#2}}{\mathbb{E}_{#1}}{%
\ifthenelse{\equal{#3}{0}}{\mathbb{E}_{#1}\bracks{#2}}{\mathbb{E}_{#1}\bracks{#2 \middle| #3}}}%
}
\newcommandx{\var}[3][1, 3=0]{
\ifthenelse{\isempty{#2}}{\operatorname{Var}_{#1}}{%
\ifthenelse{\equal{#3}{0}}{\operatorname{Var}_{#1}\pars{#2}}{\operatorname{Var}_{#1}\pars{#2 \middle| #3}}}%
}
\newcommandx{\cov}[4][1, 4=0]{
\ifthenelse{\isempty{#2} \AND \isempty{#3}}{\operatorname{Cov}_{#1}}{%
\ifthenelse{\equal{#4}{0}}{\operatorname{Cov}_{#1}\pars{#2, #3}}{\operatorname{Cov}_{#1}\pars{#2, #3 \middle| #4}}}%
}
\newcommandx{\corr}[3][1]{\ifthenelse{\isempty{#2} \AND \isempty{#3}}{\operatorname{Corr}_{#1}}{\operatorname{Corr}_{#1}\pars{#2, #3}}}

% Lois usuelles de probabilités
\newcommand{\Ber}[1]{\mathcal{B}ernoulli\pars{#1}}       % Bernoulli
\newcommand{\Binom}[2]{\mathcal{B}\pars{#1, #2}}         % Binomiale
\newcommand{\Poisson}[1]{\mathcal{P}\pars{#1}}           % Poisson
\newcommand{\Geo}[1]{\mathcal{G}eo\pars{#1}}             % Géométrique
\newcommand{\Unif}[1]{\mathcal{U}nif_{#1}}               % Uniforme
\newcommand{\Exp}[1]{\mathcal{E}xp\pars{#1}}             % Exponentielle
\newcommandx{\Norm}[3][1]{\mathcal{N}_{#1}\pars{#2, #3}} % Normale
\newcommand{\Gam}[2]{\Gamma\pars{#1, #2}}                % Gamma
\newcommand{\Betaloi}[2]{\beta\pars{#1, #2}}             % Beta
\newcommand{\Pareto}[2]{\mathcal{P}areto\pars{#1, #2}}   % Pareto
\newcommand{\Laplace}[1]{\mathcal{L}\pars{#1}}           % Laplace
\newcommand{\Cauchy}[1]{\mathcal{C}\pars{#1}}            % Cauchy

% Égalités
\newcommandx{\egalloi}{\overset{\mathrm{\mathcal{L}oi}}{=}} % égalité en loi
\newcommandx{\egalprob}{\overset{\mathbb{P}}{=}}            % égalité en probabilité
\newcommandx{\egaltxt}[1]{\overset{\mathrm{#1}}{=}}         % égal avec overscript
\newcommandx{\simiid}{\overset{\mathrm{iid}}{\sim}}         % sim iid

% Indicatrice
\newcommand{\1}[1][]{\mathds{1}_{#1}}

% max, min, argmax et argmin avec subscript
\newcommandx{\maxx}[1]{\underset{#1}{\max}}
\newcommandx{\minn}[1]{\underset{#1}{\min}}
\newcommandx{\argmax}[1][1]{\underset{#1}{\arg\max}}
\newcommandx{\argmin}[1][1]{\underset{#1}{\arg\min}}

% matrice 3*3 diagonale avec la diagonale donnée sur les 3 arguments
\newcommand{\mattroisdiag}[3]{\left( \begin{array}{ccc} #1 &  0 &  0 \\ 0  & #2 &  0 \\ 0  &  0 & #3\end{array} \right)}

% Intégration
\newcommand{\dint}{\mathrm{d}}
\newcommandx{\integ}[4][2]{\int_{#1}^{#2} #3 \, \mathrm{d} #4} 

% moyenne simple et quadratique d'une grandeur scalaire
\newcommand{\moy}[1]{\overline{#1}}
\newcommand{\moyy}[1]{\overline{#1^2}}

% Vecteurs
\let\vecteur\overrightarrow % Permet de modifier la taille de la flèche d'un vecteur quand ce dernier est composé de plusieurs lettres par exemple.
\newcommand*\coord[2]
{
   \vecteur{#1} \,
   \begin{pmatrix}
      #2
   \end{pmatrix}
} % Permet de déclarer les coordonnées d'un vecteur, exemple : \[\coord{AB}{12\\21} \coord{BC}{21\\12\\32}\]

% Surface et volume
\newcommandx{\surf}[2][2=m]{\numprint{#1}\,#2\textsuperscript{2}}
\newcommandx{\vol}[2][2=m]{\numprint{#1}\,#2\textsuperscript{3}}

% Fonction
\newcommand*\fonction[5]{
#1 \colon \left\{\begin{alignedat}{2}  &#2 &\: &\to      #3\\
                                &#4 &   &\mapsto  #5
\end{alignedat} \right. \kern-\nulldelimiterspace} % Permet de déclarer facilement une fonction, exemple : $\fonction{f}{E}{F}{x}{f(x)}$

% Autres commandes utiles
\newcommand{\compos}{\circ}                 % operateur de composition de fonctions
\DeclareMathOperator{\card}{card}           % On déclare l’opérateur \card qui correspond à « card ».
\newcommand*\PI{\ensuremath{\pi}}           % Permet d'afficher pi que l'on soit en mode math ou non.
\newcommand{\ds}[1]{\displaystyle{#1}}      % Force LaTeX à gérer les indices et les exposants comme si il était en mode mathématique isolé
\newcommand{\kronecker}[0]{\mathrm{\delta}} % symbole de Kronecker
\newcommand{\heaviside}[0]{\mathrm{H}}      % fonctions d'Heaviside
\newcommand{\dirac}[0]{\mathrm{\delta}}     % Distribution de Dirac



==> preambule/commandes_typo.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Ce fichier contient des commandes pour respecter
% la typographie française, mais également pour 
% les abréviations.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Évite veuves et orphelines
\widowpenalty=10000
\clubpenalty=10000 

% Permet de modifier l'espace entre es lignes.
\renewcommand{\baselinestretch}{1.1} 
\onehalfspacing % Permet de mettre le reste du texte avec un interligne de 1,5 (recommandé pour les articles universitaires).

% Chiffres romain
\newcommand{\cRM}[1]{\MakeUppercase{\romannumeral #1}}
% Capital
\newcommand{\cRm}[1]{\textsc{\romannumeral #1}}
% Petit majuscule
\newcommand{\crm}[1]{\romannumeral #1} % Minuscule

% Siècle
\newcommand*{\siecle}[1]{%
\ifnum #1=1%
\cRm{#1}\textsuperscript{er}~siècle%
\else%
\cRm{#1}\textsuperscript{e}~siècle%
\fi%
}%
\newcommand*{\siecles}[2]{\cRm{#1}~-~\cRm{#2}\textsuperscript{e}~siècles}

% Guillements
\newcommand{\guill}[1]{\og #1\fg{}}

% Nom d'auteur 
\newcommand\auteur[2]{#1~\textsc{#2}\xspace}

% Abréviations
\newcommand{\ssi}{si et seulement si\xspace}
\newcommand{\cad}{c'est-à-dire\xspace}
\newcommand{\cf}[0]{\textit{cf.}\xspace} % Cf. avec espace à la suite
\newcommand{\apjc}{apr. J.-C.\xspace} % après Jésus-Christ
\newcommand{\avjc}{av. J.-C.\xspace} % avant Jésus-Christ
\newcommand{\Mme}{M\textsuperscript{me}\xspace} % Madame
\newcommand{\Mlle}{M\textsuperscript{lle}\xspace} % Mademoiselle
\newcommand{\numero}{n\textsuperscript{o}\xspace} % numéro
\newcommand{\Num}{N\textsuperscript{o}\xspace} % Numéro
\newcommand{\nums}{n\textsuperscript{os}\xspace} % numéros
\newcommand{\Nums}{N\textsuperscript{os}\xspace} % Numéros




